Entity-Based Evaluation of Political Bias in Automatic Summarization

Growing literature has shown that NLP systems may encode social biases; however, the political bias of summarization models remains relatively unknown. In this work, we use an entity replacement method to investigate the portrayal of politicians in automatically generated summaries of news articles. We develop an entity-based computational framework to assess the sensitivities of several extractive and abstractive summarizers to the politicians Donald Trump and Joe Biden. We find consistent differences in these summaries upon entity replacement, such as reduced emphasis of Trump's presence in the context of the same article and a more individualistic representation of Trump with respect to the collective US government (i.e., administration). These summary dissimilarities are most prominent when the entity is heavily featured in the source article. Our characterization provides a foundation for future studies of bias in summarization and for normative discussions on the ideal qualities of automatic summaries.

==> additional_replacements.tex <==

\section{Additional Replacements}
\label{app:replacements}

\begin{table}
    \centering
    \small
    \begin{tabular}{p{1.5cm} p{0.5cm} p{0.6cm}p{0.5cm} p{0.5cm} p{0.6cm} p{0.5cm}}
        \toprule
        {$e_1$} &\multicolumn{3}{c}{Trump} &         \multicolumn{3}{c}{Biden}   \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7}
        {$e_2$} &    Biden &                                   Obama &                          Bush &                                    Trump &                                   Obama &                                   Bush \\
        \midrule
        \PreSumm             &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ &                      $\uparrow$$\uparrow$ &                                       \textemdash &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ &              $\downarrow$$\downarrow$$\downarrow$ \\
        \PEGASUS &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &          $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ \\
        \BART        &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &          $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ &              $\downarrow$$\downarrow$$\downarrow$ &          $\uparrow$$\uparrow$$\uparrow$$\uparrow$ \\
        \ProphetNet  &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &          $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ &          $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &          $\uparrow$$\uparrow$$\uparrow$$\uparrow$ \\
        \bottomrule
        \end{tabular}
        \caption{\label{tab:all_freqs} 
		Trump is less likely to be mentioned in abstractive summaries than the other presidents, which may skew reader perception of the event.
        \karen{extra}
		}
\end{table}


\begin{table*}
    \small
    \centering
    \begin{tabular}{lllllllllllll}
        \toprule
        {$e_1$} & \multicolumn{6}{c}{Trump} & \multicolumn{6}{c}{Biden}  \\
        \cmidrule(lr){2-7} \cmidrule(lr){8-13}
        {$e_2$} & \multicolumn{2}{c}{Biden} & \multicolumn{2}{c}{Obama} & \multicolumn{2}{c}{Bush} & \multicolumn{2}{c}{ Trump} & \multicolumn{2}{c}{Obama} & \multicolumn{2}{c}{Bush} \\
        {} &                                        20 &                                        21 &                    20 &           21 &                              20 &           21 &                                    20 &                                    21 &                                    20 &                                    21 &                                    20 &                                                21 \\
        \midrule
        \PreSumm             &                      $\uparrow$$\uparrow$ &                      $\uparrow$$\uparrow$ &           \textemdash &  \textemdash &                     \textemdash &  \textemdash &  $\downarrow$$\downarrow$$\downarrow$ &                           \textemdash &  $\downarrow$$\downarrow$$\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$ &              $\downarrow$$\downarrow$ &                                      $\downarrow$ \\
        \PEGASUS &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &           \textemdash &  \textemdash &                    $\downarrow$ &  \textemdash &  $\downarrow$$\downarrow$$\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$ &              $\downarrow$$\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ \\
        \BART        &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &            $\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$ &  \textemdash &  $\uparrow$$\uparrow$$\uparrow$ &  \textemdash &              $\downarrow$$\downarrow$ &                          $\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$ &              $\downarrow$$\downarrow$ &                            $\uparrow$ &                                       \textemdash \\
        \ProphetNet  &            $\uparrow$$\uparrow$$\uparrow$ &            $\uparrow$$\uparrow$$\uparrow$ &           \textemdash &  \textemdash &                    $\downarrow$ &  \textemdash &  $\downarrow$$\downarrow$$\downarrow$ &              $\downarrow$$\downarrow$ &              $\downarrow$$\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$ &              $\downarrow$$\downarrow$$\downarrow$ \\
        \bottomrule
        \end{tabular}
        \caption{\label{tab:all_vice} 
		Biden is more likely to be associated with ``Vice President'' in all cases. 
        \karen{extra}
		}
\end{table*}


\begin{table*}
    \centering
    \small
    \begin{tabular}{lllllllllllll}
        \toprule
        {$e_1$} & \multicolumn{6}{c}{Trump} & \multicolumn{6}{c}{Biden}  \\
        \cmidrule(lr){2-7} \cmidrule(lr){8-13}
        {$e_2$} & \multicolumn{2}{c}{Biden} & \multicolumn{2}{c}{Obama} & \multicolumn{2}{c}{Bush} & \multicolumn{2}{c}{ Trump} & \multicolumn{2}{c}{Obama} & \multicolumn{2}{c}{Bush} \\
        {} &                                        20 &                                    21 &                                        20 &                              21 &                                        20 &                              21 &           20 &                                                21 &           20 &                              21 &                                    20 &                                                21 \\
        \midrule
        \PreSumm             &      $\downarrow$$\downarrow$$\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$ &                              $\downarrow$ &                    $\downarrow$ &            $\uparrow$$\uparrow$$\uparrow$ &                     \textemdash &  \textemdash &          $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  \textemdash &  $\uparrow$$\uparrow$$\uparrow$ &                           \textemdash &          $\uparrow$$\uparrow$$\uparrow$$\uparrow$ \\
        \PEGASUS &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &        $\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &                     \textemdash &  \textemdash &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ &  \textemdash &                    $\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$ &              $\downarrow$$\downarrow$$\downarrow$ \\
        \BART       &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &        $\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$ &  \textemdash &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ &  \textemdash &                     \textemdash &                           \textemdash &                    $\uparrow$$\uparrow$$\uparrow$ \\
        \ProphetNet  &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &        $\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$ &  $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &            $\uparrow$$\uparrow$ &  \textemdash &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ &  \textemdash &  $\uparrow$$\uparrow$$\uparrow$ &                          $\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ \\
        \bottomrule
        \end{tabular}
        \caption{\label{tab:all_admin} 
		Trump is less likely to appear with the word ``administration'' in all abstractive summaries, suggesting a less unified view of him
        with respect to the US government than the other presidents.
        \karen{extra}
		}
\end{table*}






==> entities.tex <==


\begin{table*}[t]
    \small
        \centering
        \setlength\extrarowheight{2pt} 
        \begin{tabular}{ m{3cm} | p{1cm} | p{1cm}|  p{1cm} | p{1cm}|  p{1cm} | p{1cm}|  p{1cm} | p{1cm} }
            \toprule
            {Party Name} &\multicolumn{2}{c|}{\PreSumm{}} &         \multicolumn{2}{c|}{\PEGASUS}  &               \multicolumn{2}{c|}{\BART}  & \multicolumn{2}{c}{\ProphetNet}  \\
            \cline{2-9}
            {}   & T$\to$B & B$\to$T &  T$\to$B & B$\to$T &  T$\to$B & B$\to$T & T$\to$B & B$\to$T   \\
            \hline
            \DEM  &                           \textemdash &                               \textemdash &                               \textemdash &                                       \textemdash &                               \textemdash &                              $\uparrow$$\uparrow$ &                               \textemdash &                                       \textemdash \\
\REP  &  $\downarrow$$\downarrow$$\downarrow$ &                                $\uparrow$ &                              $\downarrow$ &                                       \textemdash &                               \textemdash &                                       \textemdash &      $\downarrow$$\downarrow$$\downarrow$ &                                       \textemdash \\
\bottomrule
        \end{tabular}
        \caption{Summaries demonstrate more significant differences in mentioning \REP than \DEM party names.
        }
        \label{tab:dem_reps} 
\end{table*}
   

\subsection{Co-occurring Political Entities} 
\label{sec:co_pols}

Next, we examine co-occurring politicians with a focus along the partisan separations.



\para{Measurement:} 
We start by considering the frequency of direct mentions of \emph{party names} of 
Democrats (\DEM $=$ \{``Democrat(s)'', ``Democratic''\}) and Republicans (\REP $=$ \{``Republican(s)'', ``GOP''\})
in the summaries. 
In addition, we extract the mentions of other US political figures in the summaries and track their genders and party affiliations.
This information about US senators, representatives, and governors are obtained from CivilServiceUSA.\footnote{\href{https://github.com/CivilServiceUSA/}{https://github.com/CivilServiceUSA/}. Only male and female labels are distinguished in this resource, but the framework is extendable to gender identities of non-binary nature.} 
Example summary pairs can be found in Appendix \ref{app:ex}.


\para{Summaries demonstrate more significant differences in mentions of \REP than \DEM.} 
Table~\ref{tab:dem_reps} shows that there rarely exists significant differences in mentions of \DEM party names: only \BART summaries become more likely to mention the Democratic party when replacing Biden with Trump.
In comparison,
for \PreSumm, \PEGASUS, and \ProphetNet, Biden is associated with fewer %
\REP than Trump, suggesting a partisan bias.   




\begin{table*}[t]
    \small
	\centering
    \setlength\extrarowheight{2pt} 
    \begin{tabular}{ m{3cm} | p{1cm} | p{1cm}|  p{1cm} | p{1cm}|  p{1cm} | p{1cm}|  p{1cm} | p{1cm} }
        \toprule
        {Politician Attribute} &\multicolumn{2}{c|}{\PreSumm{}} &         \multicolumn{2}{c|}{\PEGASUS}  &               \multicolumn{2}{c|}{\BART}  & \multicolumn{2}{c}{\ProphetNet}  \\
        \cline{2-9}
        {}   & T$\to$B & B$\to$T &  T$\to$B & B$\to$T &  T$\to$B & B$\to$T & T$\to$B & B$\to$T   \\
        \hline
        democrat    &  $\downarrow$$\downarrow$$\downarrow$ &  $\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$ &             $\uparrow$ &     \textemdash &     \textemdash &           \textemdash &           \textemdash \\
        republican  &  $\downarrow$$\downarrow$$\downarrow$ &  $\uparrow$$\uparrow$ &              $\downarrow$$\downarrow$ &            \textemdash &     \textemdash &     \textemdash &            $\uparrow$ &           \textemdash \\
        independent &                           \textemdash &           \textemdash &                           \textemdash &            \textemdash &     \textemdash &     \textemdash &           \textemdash &           \textemdash \\
\hline
male        &  $\downarrow$$\downarrow$$\downarrow$ &  $\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$ &   $\uparrow$$\uparrow$ &     \textemdash &     \textemdash &           \textemdash &           \textemdash \\
female      &                           \textemdash &           \textemdash &                           \textemdash &            \textemdash &    $\downarrow$ &     \textemdash &           \textemdash &           \textemdash \\
\bottomrule
    \end{tabular}
    \caption{Trump summaries from \PreSumm and \PEGASUS include more politicians by name that are male, in the Democratic party, and/or in the Republican party.}
    \label{tab:co_pols} 
\end{table*}



\para{Biden summaries tend to include fewer names of other politicians.}
The difference between parties is less clear for co-occurring politicians.
Biden summaries from \PreSumm and \PEGASUS models include fewer politicians in both the Democratic Party and the Republican Party, as shown in \tbref{tab:co_pols}.
It is possible that the direct name references emphasize Trump's political alliances and rivalries more strongly. 
Biden summaries tend to also have fewer male politicians than the corresponding ones of Trump in \PreSumm and \PEGASUS. 
Since most US politicians are identified as male (at the time of this paper's writing), we hypothesize that summaries about Biden would include fewer co-occurring politician names in general. 







 


        
       
    






    
    
    




    
    
    


==> lexical.tex <==








\begin{table*}[t]
    \small
        \centering
        \setlength\extrarowheight{2pt} 
        \begin{tabular}{ l | p{1cm} | p{1cm}|  p{1cm} | p{1cm}|  p{1cm} | p{1cm}|  p{1cm} | p{1cm} }
            \toprule
            {Lexicon} &\multicolumn{2}{c|}{\PreSumm{}} &         \multicolumn{2}{c|}{\PEGASUS}  &               \multicolumn{2}{c|}{\BART}  & \multicolumn{2}{c}{\ProphetNet}  \\
            \cline{2-9}
            {}   & T$\to$B & B$\to$T &  T$\to$B & B$\to$T &  T$\to$B & B$\to$T & T$\to$B & B$\to$T   \\
            \hline
            assertives &   $\uparrow$ &  \textemdash &            \textemdash &               \textemdash &  $\uparrow$$\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$ &            $\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$ \\
            factives   &  \textemdash &  \textemdash &            \textemdash &                $\uparrow$ &                     \textemdash &                            $\uparrow$ &                     \textemdash &                           \textemdash \\
            report verbs    &  \textemdash &  \textemdash &   $\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$ &  $\uparrow$$\uparrow$$\uparrow$ &                           \textemdash &  $\uparrow$$\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$ \\
            hedges     &  \textemdash &  \textemdash &            \textemdash &               \textemdash &                     \textemdash &                           \textemdash &                     \textemdash &                           \textemdash \\        
            \bottomrule
        \end{tabular}
        \caption{\label{lexicons} Abstractive summaries are more sensitive to entity replacement with regards to linguistic markers of author bias. Specifically, these models tend to use more such markers for Biden than Trump.
        }
\end{table*}
      

\subsection{Linguistics Markers of Author Bias}

We then apply the methods of \citet{patel-pavlick-2021-stated} to examine linguistic markers of author bias.

\para{Measurement:} 
We assess the prevalence of words that indicate subjective assessments of the speakers (e.g., ``Trump claimed'').
Specifically, we consider the following categories: 
\begin{itemize}[leftmargin=*,itemsep=-2pt,topsep=0pt]
    \item \textbf{Assertives}: verbs with complement clauses asserting a proposition, with varying degree of certainty (e.g., \textit{claim}, \textit{allege}); we use Hooper's lexicon of 67 assertive verbs \citep{hooper_assertive_1975}.
    \item \textbf{Factives}: verbs presupposing the truth of their complement clause, often representing a person’s stance (e.g., \textit{reveal}, \textit{realize}); we use Hooper's lexicon of 98 factives \citep{hooper_assertive_1975}.
    \item \textbf{Report verbs}: verbs indicating that discourse is being quoted or paraphrased (e.g., \textit{observed}, \textit{testified}); we use the lexicon from \citet{recasens_linguistic_2013} containing 180 report verbs.
    \item \textbf{Hedges}: words reducing one’s commitment to the truth of a proposition (e.g., \textit{maybe}, \textit{apparently});
     we use the lexicon from \citet{tan+lee:16} with 255 hedging regular expressions.
\end{itemize}




\para{Abstractive summaries for Biden tend to contain more markers of author bias.} 
Table~\ref{lexicons} shows little difference in linguistic markers of author bias for \PreSumm, and no difference in hedges across all models.
However, all abstractive summaries demonstrate some biases in the other three categories.
Different from LIWC, \ProphetNet and \BART, the models {\em not} designed specifically for summarization, exhibit more salient biases. 
For example, \ProphetNet tend to include more assertives and report verbs in Biden summaries.



Note that counting the frequency does not differentiate whether Biden uses hedges himself, or someone else uses hedges on claims about Biden.



\subsection{Psychological Meaning in LIWC} 
\label{ssec:liwc}

Finally, we examine biases based on lexicons as outined in LIWC \citep{LIWC2007}.

\para{Measurement:}
We consider three psychological processes, and corresponding sub-categories, that are relevant in the political context: affective processes, cognitive processes, and social processes.\footnote{The other three processes are perceptual processes, biological processes, and relativity.}
The feature function here is the frequency of lexicons in each category that occur in the summaries.
We present these results in \tbref{full_liwc}.

\begin{table*}
	\small
		\centering
		\setlength\extrarowheight{2pt} 
		\begin{tabular}{ m{3cm} | p{1cm} | p{1cm}|  p{1cm} | p{1cm}|  p{1cm} | p{1cm}|  p{1cm} | p{1cm} }
			\toprule
			{LIWC Category} &\multicolumn{2}{c|}{\PreSumm{}} &         \multicolumn{2}{c|}{\PEGASUS}  &               \multicolumn{2}{c|}{\BART}  & \multicolumn{2}{c}{\ProphetNet}  \\
			\cline{2-9}
			{}   & T$\to$B & B$\to$T &  T$\to$B & B$\to$T &  T$\to$B & B$\to$T & T$\to$B & B$\to$T   \\
			\hline
			\textbf{Affective processes}  &  $\uparrow$$\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$ &                    $\uparrow$$\uparrow$$\uparrow$ &                                       \textemdash &                  $\uparrow$$\uparrow$ &                                       \textemdash &                           \textemdash &                           \textemdash \\
			Positive emotions  &            $\uparrow$$\uparrow$ &              $\downarrow$$\downarrow$ &                                       \textemdash &                                       \textemdash &                  $\uparrow$$\uparrow$ &                                       \textemdash &                           \textemdash &                           \textemdash \\
			Negative emotions  &  $\uparrow$$\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$ &                    $\uparrow$$\uparrow$$\uparrow$ &                                       \textemdash &                           \textemdash &                                       \textemdash &                           \textemdash &                           \textemdash \\
			Anger   &  $\uparrow$$\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$ &                    $\uparrow$$\uparrow$$\uparrow$ &                                       \textemdash &                           \textemdash &                                       \textemdash &                           \textemdash &                           \textemdash \\
			Anxiety     &                      $\uparrow$ &                           \textemdash &                                       \textemdash &                                       \textemdash &                           \textemdash &                                       \textemdash &                           \textemdash &                           \textemdash \\
			Sadness     &                     \textemdash &                           \textemdash &                              $\uparrow$$\uparrow$ &                                       \textemdash &                           \textemdash &                                       \textemdash &                           \textemdash &                           \textemdash \\
			\hline
			\textbf{Cognitive processes} &                    $\downarrow$ &                           \textemdash &              $\downarrow$$\downarrow$$\downarrow$ &                    $\uparrow$$\uparrow$$\uparrow$ &                           \textemdash &                                      $\downarrow$ &                           \textemdash &                           \textemdash \\
			Insight &                    $\downarrow$ &                           \textemdash &              $\downarrow$$\downarrow$$\downarrow$ &                              $\uparrow$$\uparrow$ &                           \textemdash &                                       \textemdash &                           \textemdash &                           \textemdash \\
			Causation  &                     \textemdash &              $\downarrow$$\downarrow$ &              $\downarrow$$\downarrow$$\downarrow$ &                              $\uparrow$$\uparrow$ &                           \textemdash &                                       \textemdash &                           \textemdash &                           \textemdash \\
			Discrepancy &                    $\downarrow$ &                           \textemdash &              $\downarrow$$\downarrow$$\downarrow$ &                              $\uparrow$$\uparrow$ &                           \textemdash &                                       \textemdash &                           \textemdash &                           \textemdash \\
			Inhibition   &                     \textemdash &                           \textemdash &                    $\uparrow$$\uparrow$$\uparrow$ &                                       \textemdash &        $\uparrow$$\uparrow$$\uparrow$ &                                       \textemdash &                           \textemdash &                           \textemdash \\
			Tentative  &                     \textemdash &                           \textemdash &              $\downarrow$$\downarrow$$\downarrow$ &                                       \textemdash &                           \textemdash &                                       \textemdash &                           \textemdash &                           \textemdash \\
			Certainty &                    $\downarrow$ &                           \textemdash &                                      $\downarrow$ &                                       \textemdash &                           \textemdash &                                       \textemdash &                           \textemdash &                           \textemdash \\
			Inclusive   &                     \textemdash &                          $\downarrow$ &              $\downarrow$$\downarrow$$\downarrow$ &                    $\uparrow$$\uparrow$$\uparrow$ &                           \textemdash &                              $\uparrow$$\uparrow$ &              $\downarrow$$\downarrow$ &                           \textemdash \\
			Exclusive    &                     \textemdash &                          $\downarrow$ &  $\downarrow$$\downarrow$$\downarrow$$\downarrow$ &          $\uparrow$$\uparrow$$\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$ &                    $\uparrow$$\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$ &        $\uparrow$$\uparrow$$\uparrow$ \\
			\hline
			\textbf{Social processes}  &  $\uparrow$$\uparrow$$\uparrow$ &  $\downarrow$$\downarrow$$\downarrow$ &                                       \textemdash &                              $\uparrow$$\uparrow$ &                           \textemdash &                                       \textemdash &                           \textemdash &                            $\uparrow$ \\
			Friends &                      $\uparrow$ &                           \textemdash &                                       \textemdash &                          $\downarrow$$\downarrow$ &                           \textemdash &                                       \textemdash &                           \textemdash &                           \textemdash \\
			Family  &                     \textemdash &                           \textemdash &                              $\uparrow$$\uparrow$ &                                       \textemdash &                           \textemdash &                                       \textemdash &        $\uparrow$$\uparrow$$\uparrow$ &                          $\downarrow$ \\
			Humans  &                     \textemdash &                           \textemdash &                                       \textemdash &                                       \textemdash &                           \textemdash &                                       \textemdash &                            $\uparrow$ &                           \textemdash \\
			
			\bottomrule
		\end{tabular}
		\caption{\label{full_liwc} 
		\PreSumm and \PEGASUS summaries see significant changes in psychological process lexicons when replacing entities in the source article. In particular, \PreSumm is sensitive  in affective processes, while \PEGASUS is sensitive in cognitive processes. 
		}
\end{table*}

\para{Models specifically designed for summarization tend to exhibit more biases with respect to LIWC words.}
Both \PreSumm and \PEGASUS show some biases in all the three categories, while \BART and \ProphetNet show fewer differences.
When replacing Trump with Biden, summaries for Biden include more words indicating affective processes.
Specifically, \PreSumm and \BART produce Biden summaries with more positive words; \PreSumm and \PEGASUS also produce Biden summaries with more negative words. 


We also note consistently strong differences in words about cognitive processes with \textsc{PEGASUS} summaries. 
In particular, summaries for Biden contain less inclusive words (like \textit{with} and \textit{include}) and less exclusive words (like \textit{without} and \textit{but}), which could be related to making associations with other people; this echoes our previous result that Biden is mentioned with fewer politicians than Trump.











